Homotopy theory of symmetric powers

We introduce the symmetricity notions of symmetric h-monoidality, symmetroidality, and symmetric flatness. As shown in our paper arXiv:1410.5675, these properties lie at the heart of the homotopy theory of colored symmetric operads and their algebras. In particular, the former property can be seen as the analog of Schwede and Shipley's monoid axiom for algebras over symmetric operads and allows one to equip categories of such algebras with model structures, whereas the latter ensures that weak equivalences of operads induce Quillen equivalences of categories of algebras. We discuss these properties for elementary model categories such as simplicial sets, simplicial presheaves, and chain complexes. Moreover, we provide powerful tools to promote these properties from such basic model categories to more involved ones, such as the stable model structure on symmetric spectra.

==> biblio <==
AguiarMahajan:Monoidal MR2724388 Zbl:1209.18002 doi:10.1090/crmm/029 https://pi.math.cornell.edu/~maguiar/a.pdf
Amrani:Model MR3313635 Zbl:06419552 doi:10.1007/s40062-013-0041-8 arXiv:1110.2695
Barnes:Splitting MR2494375 Zbl:1163.55002 arXiv:0812.0313v1 doi:10.1016/j.jpaa.2008.10.004
BarrWells:Toposes MR2178101 Zbl:1081.18006 http://tac.mta.ca/tac/reprints/articles/12/tr12abs.html
Barwick:Left MR2771591 Zbl:1243.18025 arXiv:0708.2067 doi:10.4310/hha.2010.v12.n2.a9
BataninBerger:Homotopy arXiv:1305.0086v6
BauesJibladzeTonks:Cohomology MR1436920 Zbl:0860.18006
BayehHessKarpovaKedziorekRiehlShipley:Left MR3380069 Zbl:1346.18023 arXiv:1401.3651v2 doi:10.1090/conm/641/12859
Behrend:Differential arXiv:math/0212225
Beilinson:Higher MR760999 Zbl:03944014
BergerMoerdijk:Axiomatic MR2016697 Zbl:1041.18011 arXiv:math/0206094 doi:10.1007/s00014-003-0772-y
BergerMoerdijk:Boardman MR2248514 Zbl:1105.18007 arXiv:math/0502155 doi:10.1016/j.top.2006.05.001
BergerMoerdijk:Derived MR2527612 Zbl:1171.18005 arXiv:0801.2664v2
BergerMoerdijk:Homotopy MR3094501 Zbl:1282.18006 arXiv:1201.2134v3 doi:10.1093/qmath/hat023
BergerMoerdijk:Resolution MR2342815 Zbl:1134.18005 arXiv:math/0512576v2 doi:10.1090/conm/431/08265
Bergner:Model MR2276611 Zbl:1114.18006 arXiv:math/0406507v2 doi:10.1090/S0002-9947-06-03987-0
Borceux:1 MR1291599 Zbl:1143.18001 doi:10.1017/cbo9780511525858 gen:3D413ACEB21BD494E24D778E74F5438D
Borceux:2 MR1313497 Zbl:1143.18002 doi:10.1017/cbo9780511525865 gen:25437F068C15E3852CE4583EEACC7367
Caviglia:Model arXiv:1401.6983v1
ChacholskiScherer:Homotopy MR1879153 Zbl:1006.18015 arXiv:math/0110316v1
CisinskiDeglise:Local MR2529161 Zbl:1175.18007 arXiv:0712.3296v1
CisinskiDeglise:Triangulated arXiv:0912.2110v3
CisinskiMoerdijk:Dendroidal MR3100888 Zbl:1291.55005 arXiv:1109.1004v1 doi:10.1112/jtopol/jtt006
Cole:Mixing MR2203016 Zbl:1094.55015
Crans:Quillen MR1346427 Zbl:0828.18005
Deninger:Higher MR1329043 Zbl:0847.55014
Dugger:Combinatorial MR1870516 Zbl:1001.18001 arXiv:math/0007068v1
DuggerHollanderIsaksen:Hypercovers MR2034012 Zbl:1045.55007 arXiv:math/0205027v2
DwyerKan:Singular MR0749528 Zbl:0555.55019 doi:10.1016/1385-7258(84)90016-7
DwyerHirschhornKanSmith:Homotopy MR2102294 Zbl:1072.18012 doi:10.1090/surv/113 gen:77C0EAED9EB053F0220F11769BAEA50A
ElmendorfKrizMandellMay:Rings MR1417719 Zbl:0894.55001 gen:EFF9E7553C7E3FF742A74F7009922D2A
ElmendorfMandell:Rings MR2254311 Zbl:1117.19001 arXiv:math/0403403
EsnaultViehweg:Deligne MR0944991 Zbl:0656.14012 https://page.mi.fu-berlin.de/esnault/preprints/ec/deligne_beilinson.pdf
Fresse:Modules MR2494775 Zbl:1178.18007 arXiv:0704.3090v4
Gambino:Weighted MR2586997 Zbl:1228.18013
GambinoJoyal:Operads arXiv:1405.7270
GepnerHaugseng:Enriched MR3345192 Zbl:1342.18009 doi:10.1016/j.aim.2015.02.007 arXiv:1312.3178
GoerssHopkins:Commutative MR2125040 Zbl:1086.55006 https://math.northwestern.edu/~pgoerss/papers/sum.pdf
GoerssHopkins:Structured https://math.northwestern.edu/~pgoerss/spectra/obstruct.pdf Paul G. Goerss, Michael J. Hopkins: Moduli problems for structured ring spectra (June~8, 2005)
GoerssJardine:Simplicial MR1711612 Zbl:0949.55001 gen:7260527709E3924EAAC4DA2C062725AD
GorchinskiyGuletskii:Positive arXiv:1108.3509v3 doi:10.1007/s10485-016-9480-9
GorchinskiyGuletskii:Symmetric arXiv:0907.0730 MR3464032 Zbl:06548176 arXiv:0907.0730v4 doi:10.1016/j.aim.2016.01.011
Guillou:Short https://faculty.math.illinois.edu/~bertg/EquivModels.pdf Bert Guillou: A short note on models for equivariant homotopy theory
GutierrezVogt:Model MR2875831 Zbl:1248.18010 arXiv:1006.2316v2 doi:10.1007/s00209-010-0794-2
HarpazNuitenPrasma arXiv:1612.02607v2 doi:10.1007/s11856-019-1933-z
Harper:Corrigendum MR3342691 Zbl:1315.55006 doi:10.2140/agt.2015.15.1229 arXiv:0801.0193v4
Harper:Monoidal MR2593672 Zbl:1231.55011 arXiv:0801.0191
Harper:Symmetric MR2539191 Zbl:1235.55004 arXiv:0801.0193v3
HarperHess:Homotopy MR3073927 Zbl:1270.18025 arXiv:1102.1234v5
HessShipley:Waldhausen doi:10.1016/j.aim.2015.12.019 arXiv:1402.4719v2
Hinich:Homological MR1465117 Zbl:0894.18008 arXiv:q-alg/9702015 doi:10.1080/00927879708826055
Hirschhorn:Model MR1944041 Zbl:1017.55001 doi:10.1090/surv/099 gen:23EF8741E363DBAE39D1E7BA13F134E6
HolmstromScholbach:Arakelov doi:10.1090/jag/648 arXiv:1012.2523
HopkinsQuick:Hodge MR3335251 Zbl:06417723 arXiv:1212.2173v3 doi:10.1112/jtopol/jtu021
Hornbostel:Preorientations MR3116300 Zbl:1281.55009 arXiv:1005.4546 doi:10.2140/agt.2013.13.2667
Hovey:Homotopy MR2066503 Zbl:1067.18012 arXiv:math/0301229
Hovey:Model MR1650134 Zbl:0909.55001 gen:229756633EF1A320BED3109B1AC1AB52 doi:10.1090/surv/063
Hovey:Smith arXiv:1401.2850
Hovey:Spectra MR1860878 Zbl:1008.55006 arXiv:math/0004051
HoveyShipleySmith:Symmetric MR1695653 Zbl:0931.55006 arXiv:math/9801077
Isaksen:Flasque MR2275013 Zbl:1116.18008 arXiv:math/0401132
Jardine:Motivic MR1787949 Zbl:0969.19004 https://www.emis.de/journals/DMJDMV/vol-05/15.html
Jardine:Simplicial MR0906403 Zbl:0624.18007
Joyal:Notes https://math.uchicago.edu/~may/IMA/JOYAL/Joyal.pdf Andr\'e Joyal: Notes on logoi
Joyal:Weak https://ncatlab.org/joyalscatlab/published/Weak+factorisation+systems Andr\'e Joyal: Weak factorisation systems
Kelly:Operads MR2177746 Zbl:1082.18009 http://tac.mta.ca/tac/reprints/articles/13/tr13abs.html
Kelly:Unified MR0589937 Zbl:0437.18004 doi:10.1017/s0004972700006353
KellyLack:Cat MR1870617 Zbl:1003.18008
Kro:Model MR2366955 Zbl:1137.18006 arXiv:math/0703838v1 doi:10.4310/hha.2007.v9.n2.a14
Lewis:Is MR1124786 Zbl:0727.55005 doi:10.1016/0022-4049(91)90030-6
LewisMandell:Modules MR2320005 Zbl:1123.18010 arXiv:math/0606275v1 doi:10.1016/j.jpaa.2006.10.002
Linton:Coequalizers MR0244341 Zbl:0181.02902 doi:10.1007/BFb0083082
LivernetRoitzheimWhitehouse:Derived MR3031646 arXiv:1110.5167
Lurie:HA https://www.math.ias.edu/~lurie/papers/HA.pdf Jacob Lurie: Higher algebra (September 18, 2017)
Lurie:HTT MR2522659 Zbl:1175.18001 arXiv:math/0608040 https://www.math.ias.edu/~lurie/papers/HTT.pdf
Mandell:Einfty MR1791268 Zbl:0974.55004
MandellMay:Equivariant MR1922205 Zbl:1025.55002
MandellMaySchwedeShipley:Model MR1806878 Zbl:1017.55004
May:Concise MR1702278 Zbl:0923.55001 https://math.uchicago.edu/~may/CONCISE/ConciseRevised.pdf
MayPonto:More MR2884233 Zbl:1249.55001 https://math.uchicago.edu/~may/TEAK/KateBookFinal.pdf
Moore:Semi MR0111027 Zbl:0089.18001 https://www.maths.ed.ac.uk/~v1ranick/papers/mexico.pdf
MorelVoevodsky:A1 MR1813224 Zbl:0983.14007
Muro:Corrections arXiv:1507.06644v1
Muro:Dwyer arXiv:1201.1575 MR3356766 Zbl:1317.18014 doi:10.1112/jtopol/jtu029
Muro:Homotopy arXiv:1101.1634 MR2821434 Zbl:1228.18006 doi:10.2140/agt.2011.11.1541
PavlovScholbach:Operads arXiv:1410.5675v3 doi:10.1112/topo.12008
PavlovScholbach:Spectra arXiv:1410.5699v2 doi:10.1017/S1474748017000202
PavlovScholbach:Symmetry arXiv:1510.04969v3 doi:10.4310/HHA.2018.v20.n1.a20
Pereira:Cofibrancy doi:10.4310/hha.2016.v18.n2.a7 arXiv:1410.4816v2
RaptisRosicky:Accessibility arXiv:1403.3042
Rezk:Every MR1881711 Zbl:0994.18008 arXiv:math/0003065v1 doi:10.1016/s0166-8641(01)00057-8
Rezk:Fibrations arXiv:math/9811038
Rezk:Model https://faculty.math.illinois.edu/~rezk/cat-ho.dvi Charles Rezk: A model category for categories
Rezk:Spaces MR2716655 https://faculty.math.illinois.edu/~rezk/rezk-thesis.dvi
Richter:Symmetry MR1937795 Zbl:1033.18009
Rosicky:Homotopy MR2349711 Zbl:1126.55004 arXiv:math/0509655v2 doi:10.1016/j.aim.2007.02.011
Sagave:DG-algebras MR2608191 arXiv:0711.4499
SagaveSchlichtkrull:Diagram MR2964635 Zbl:06094109 arXiv:1103.2764
Saito:Mixed MR1159259 Zbl:00066525 https://www.mathunion.org/fileadmin/ICM/Proceedings/ICM1990.1/ICM1990.1.ocr.pdf
Scholbach:SpecialL arXiv:1003.1215v3 doi:10.4310/AJM.2017.v21.n2.a2
Schreiber:Differential arXiv:1310.7930
Schwede:Spectra MR1466099 Zbl:0888.55010 doi:10.1016/s0022-4049(96)00058-8
Schwede:Symmetric https://www.math.uni-bonn.de/people/schwede/SymSpec-v3.pdf Stefan Schwede: Symmetric spectra
SchwedeShipley:Algebras MR1734325 Zbl:1026.18004 arXiv:math/9801082 doi:10.1112/s002461150001220x
SchwedeShipley:Equivalences MR1997322 Zbl:1028.55013 arXiv:math/0209342 doi:10.2140/agt.2003.3.287
SchwedeShipley:Stable MR1928647 arXiv:math/0108143 Zbl:1013.55005
Shipley:Convenient MR2066511 Zbl:1063.55006 doi:10.1090/conm/346/06300
Shipley:HZ-algebras MR2306038 arXiv:math/0209215
Spitzweck:Operads Zbl:1103.18300 https://d-nb.info/970107374/34 Markus Spitzweck: Operads, Algebras and Modules in Model Categories and Motives
Spitzweck:General arXiv:math/0101102v1
Tabuada:Erratum MR2377018
Tabuada:Homotopy doi:10.1016/j.aim.2009.01.014 arXiv:0801.4524 Zbl:1168.55008 MR2518634
Tabuada:Invariants arXiv:math/0507227 MR2196100 Zbl:1094.18006 doi:10.1155/IMRN.2005.3309
ToenVezzosi:HomotopicalII MR2394633 Zbl:1145.14003 arXiv:math/0404373
White:Model arXiv:1403.6759v2 doi:10.1016/j.jpaa.2017.03.001
White:Monoidal arXiv:1404.5197
WhiteYau:Bousfield arXiv:1503.06720 doi:10.1007/s10485-017-9489-8
Stephan:Equivariant MR3551501 Zbl:1357.18005 arXiv:1308.0856v3 doi:10.4310/hha.2016.v18.n2.a10
Isaacson:Symmetric MR2769224 Zbl:1228.18014 arXiv:0910.4948v1 doi:10.1016/j.jpaa.2010.08.001
diBrinoPistaloPoncin:Model arXiv:1505.07720v2
HottaTakeuchiTanisaki:D-modules MR2357361 Zbl:1292.00026 doi:10.1007/978-0-8176-4523-6 gen:8C2BC0EB79B6B7730FC106577972EC0D
CostelloGwilliam:Factorization MR3586504 Zbl:06653770 doi:10.1017/9781316678626 https://people.math.umass.edu/~gwilliam/vol1may8.pdf
Haugseng:Rectification MR3402334 Zbl:1327.18015 arXiv:1312.3881v3 doi:10.2140/agt.2015.15.1931
Hinich:Rectification MR3404213 Zbl:1339.18013 arXiv:1311.4130v7
JohnsonYau:Homotopy MR2559644 Zbl:1188.18007 arXiv:0906.0015v4
Muro:HomotopyII MR3158759 Zbl:1281.18001 doi:10.2140/agt.2014.14.229 arXiv:1304.6641
Robertson:Homotopy arXiv:1111.4146v1
Jardine:Intermediate MR2252262 Zbl:1107.18007 doi:10.4153/cmb-2006-040-8

